Is Everything in Order? A Simple Way to Order Sentences

The task of organizing a shuffled set of sentences into a coherent text has been used to evaluate a machine's understanding of causal and temporal relations. We formulate the sentence ordering task as a conditional text-to-marker generation problem. We present Reorder-BART (Re-BART) that leverages a pre-trained Transformer-based model to identify a coherent order for a given set of shuffled sentences. The model takes a set of shuffled sentences with sentence-specific markers as input and generates a sequence of position markers of the sentences in the ordered text. Re-BART achieves the state-of-the-art performance across 7 datasets in Perfect Match Ratio (PMR) and Kendall's tau ($\tau$). We perform evaluations in a zero-shot setting, showcasing that our model is able to generalize well across other datasets. We additionally perform several experiments to understand the functioning and limitations of our framework.

==> abstract.tex <==
The task of organizing a shuffled set of sentences into a coherent text has been used to evaluate a machine's understanding of causal and temporal relations.  We present \textbf{Re}order-\textbf{BART} (\rebart), a \emph{sentence ordering} approach %\SC{framework or approach?} 
which leverages a pre-trained Transformer-based model to identify a coherent order for a given set of shuffled sentences. We reformulate the task as a conditional text-to-marker generation setup  where the input is a set of shuffled sentences with sentence-specific markers and the output is a sequence of position markers of the sentences in the ordered text. %\SC{"position markers of text" does not make sense. Call it "position markers of the sentences in the ordered text"}. 
\rebart achieves the state-of-the-art performance across 7 datasets in Perfect Match Ratio (PMR) and Kendall's tau ($\tau$) metric. We perform evaluations in a zero-shot setting, showcasing that our model is able to generalize well across other datasets. We additionally perform a series of experiments to understand the functioning and limitations of our framework.

==> figures/performance-10.tex <==
		\begin{tabular}{c|c c c c c}
			\hline
			{Model} & Acc & PMR & $\tau$ & LCS & Rouge-S  \TBstrut\\
			\hline
			& \multicolumn{5}{c}{NIPS Abstract}  \TBstrut\\
			\hline
			B-TSort & 39.43 & 0.00 & 0.74 & 71.68 & 83.26 \Tstrut\\
			BERSON & \textbf{50.89} & \textbf{13.33} & \textbf{0.76} & \textbf{74.96} & \textbf{87.94} \\
			Ours & 40.74 & 9.09 & 0.74 & 73.33 & 81.67\\
			\hline
			& \multicolumn{5}{c}{AAN Abstract} \TBstrut\\
			\hline
			B-TSort & 36.86 & 0.00 & 0.69 & 72.01 & 78.52 \Tstrut\\
			BERSON & 47.38 &  6.90 & 0.73 & 76.53 & 86.48 \\
			Ours & \textbf{52.59} & \textbf{12.90} & \textbf{0.76} & \textbf{80.93} & \textbf{88.31} \\
			\hline
			& \multicolumn{5}{c}{NSF Abstract} \TBstrut\\
			\hline
			B-TSort & 36.86 & 0.0  & \textbf{0.69} & \textbf{78.52} & 72.01 \Tstrut\\
			BERSON & - & - & - & - & -\\
			Ours & \textbf{38.63} & \textbf{7.25} & 0.67 & 73.95 & \textbf{83.19} \\
			\hline
		\end{tabular}

==> figures/sentence-displacement.tex <==
 in 		\begin{tabular}{c|c c c| c c c}
			\hline
			{Model} & Win=1 & Win=2 & Win=3  & Win=1 & Win=2 & Win=3  \TBstrut\\
			\hline
			& \multicolumn{3}{c}{NIPS Abstract}   & \multicolumn{3}{c}{SIND} \TBstrut\\
			\hline
			B-TSort & 87.59 & 95.59 & 98.11 & 82.67 & 95.01 & 99.09 \Tstrut\\
			BERSON & 91.98 & \textbf{96.84} & \textbf{99.29} & 84.01 & 95.11 & \textbf{99.10} \Tstrut\\
			Ours & \textbf{92.33} & 96.19 & 98.26 & \textbf{86.40} & \textbf{95.18} & 98.63 \Tstrut\\
			\hline
			& \multicolumn{3}{c}{NSF Abstract}   & \multicolumn{3}{c}{AAN Abstract} \TBstrut\\
			\hline
			B-TSort & 61.41 & 75.52 & 83.87 & 90.56 & 96.78 & 98.71 \Tstrut\\
			BERSON & \textbf{70.08} & \textbf{80.29} & \textbf{86.46} & 93.31 & 97.57 & 99.09 \Tstrut\\
			Ours & 68.33 & 78.28 & 84.29 & \textbf{95.18} & \textbf{98.09} & \textbf{99.15} \Tstrut\\
			\hline
		\end{tabular}
